Joint Approximate Partial Diagonalization of Large Matrices

Given a set of $p$ symmetric (real) matrices, the Orthogonal Joint Diagonalization (OJD) problem consists of finding an orthonormal basis in which the representation of each of these $p$ matrices is as close as possible to a diagonal matrix. We argue that when the matrices are of large dimension, then the natural generalization of this problem is to seek an orthonormal basis of a certain subspace that is a near eigenspace for all the matrices in the set. We refer to this as the problem of ``partial joint diagonalization of matrices.'' The approach proposed first finds this approximate common near eigenspace and then proceeds to a joint diagonalization of the restrictions of the input matrices in this subspace. A few solution methods for this problem are proposed and illustrations of its potential applications are provided.

==> preamble.tex <==
\def\PP{\mathcal{P}}
\def\QQ{\mathcal{Q}}
\def\OO{\mathcal{O}}
\def\HH{\mathcal{H}}
\def\ttF{\texttt{F}}
\def\RR{\mathbb{R}}
\def\CC{\mathbb{C}}
\def\tF{\texttt{F}}
\def\invt{^{-T}}%
\def\inv{^{-1}}%
\def\nref#1{(\ref{#1})}
\def\tS{\tilde{S}}
\def\trace{\text{Trace}} 
\def\diag{\text{Diag}} 
\def\Off{\texttt{Off}} 

\def \MATLAB {\textsc{MatLab}}
\providecommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\xpmatrix}[1]{\begin{pmatrix} #1 \end{pmatrix}}
 
\newcommand{\eq}[1]{\begin{equation}\label{#1}}
\newcommand{\en}{\end{equation}}

\newtheorem{algor}{{\sc Algorithm}}[section]
\newenvironment{algorithm0}{\begin{algor} \sl }{ \end{algor} } 
\def\betab{\vspace{10pt}\begin{tabbing}
xxxx\=xxxx\=xxx\=xxx\=xx\=xx\=xx\=xxx\= \kill} 
\def\entab{\end{tabbing}\vspace{0.01in}}

\newenvironment{proof}{\begin{trivlist}
		       \item[]\hspace{0.3cm}{\bf Proof.}
		       \hspace{0cm} }{\hfill $\Box$
		       \end{trivlist}}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}

